FACT-E: Causality-Inspired Evaluation for Trustworthy Chain-of-Thought Reasoning

Chain-of-Thought (CoT) prompting has improved LLM reasoning, but models often generate explanations that appear coherent while containing unfaithful intermediate steps. Existing self-evaluation approaches are prone to inherent biases: the model may confidently endorse coherence even when the step-to-step implication is not valid, leading to unreliable faithfulness evaluation. We propose FACT-E, a causality-inspired framework for evaluating CoT quality. FACT-E uses controlled perturbations as an instrumental signal to separate genuine step-to-step dependence from bias-driven artifacts, producing more reliable faithfulness estimates (\textit{intra-chain faithfulness}). To select trustworthy trajectories, FACT-E jointly considers \textit{intra-chain faithfulness} and \textit{CoT-to-answer consistency}, ensuring that selected chains are both faithful internally and supportive of the correct final answer. Experiments on GSM8K, MATH, and CommonsenseQA show that FACT-E improves reasoning-trajectory selection and yields stronger in-context learning exemplars. FACT-E also reliably detects flawed reasoning under noisy conditions, providing a robust metric for trustworthy LLM reasoning.

==> main/method.tex <==
\section{Methodology Framework}

\subsection{Causal Formulation of Reasoning Step Quality}

We model reasoning as a sequential generative process governed by a structural causal model (SCM), under which the reasoning chain is conceptualized as a causal sequence. Each reasoning step $s_t$ is generated by a deterministic structural equation:

\begin{equation}
s_t = f_t(s_{<t}, q, U_t)
\end{equation}
with $U_t$ denoting an exogenous noise variable. 
To evaluate whether a given step is plausible given the prior reasoning, we assess the interventional probability $P(s_t \mid do(s_{<t}), q)$, representing the likelihood of $s_t$ under a fixed prefix of reasoning. 

\paragraph{CoT Exogeneity Assumption.} We assume that reasoning step generation is conditionally exogenous: it depends only on the prior steps and the question, not on hidden variables. Formally:
\begin{equation}
P(s_t \mid do(s_{<t}), q) = P(s_t \mid s_{<t}, q)
\end{equation}

This allows us to approximate step plausibility via standard conditional language model probabilities. %We define the overall chain-of-thought quality score as:
% \begin{equation}
% P_{\text{CoT}}(\mathbf{S}) = \frac{1}{n} \sum_{t=1}^n P(A \mid s_t, q) \cdot P(s_t \mid s_{<t}, q)
% \end{equation}


\subsection{Quantifying Reasoning Quality with \texorpdfstring{$P_{\text{CoT}}$}{PCoT}}

We define the quality of a reasoning chain $\mathbf{S} = \{s_1, s_2, \dots, s_n\}$ for a given question $q$ through the metric $P_{\text{CoT}}$, which captures whether each reasoning step $s_t$ contributes to both accurate continuation and correctness of the final answer $A$. Formally, we define:

\begin{definition}[$P_{\text{CoT}}$] The high-quality reasoning chain $\mathbf{S} = \{s_1, \dots, s_n\}$ is one where each step $s_t$ accurately predicts the next step $s_{t+1}$ and contributes to the correct final answer. This can be quantified using Bayesian probability:
\begin{equation}
P_{\text{CoT}}(\mathbf{S}) = \frac{1}{n} \sum_{t=1}^n P(A, s_t \mid \mathbf{S}_{<t}, q),
\end{equation}
where $A$ is the correct answer, $q$ is the input question, and $\mathbf{S}_{<t} = \{s_1, \dots, s_{t-1}\}$.
\end{definition}

Applying Bayes’ rule, we decompose this joint probability into two interpretable components:

\begin{equation}
P_{\text{CoT}}(s_t) = P(A, s_t \mid \mathbf{S}_{<t}, q) = P(A \mid s_t, q) \cdot P(s_t \mid do(\mathbf{S}_{<t}), q)
\end{equation}

This formulation allows us to isolate two critical aspects of reasoning:
\begin{itemize}
    \item \textbf{Correctness Term} ($P(A \mid s_t, q)$): Measures whether the step $s_t$ contributes to the correct final answer $A$.
    \item \textbf{Coherence Term} ($P(s_t \mid do(\mathbf{S}_{<t}), q)$): Captures whether $s_t$ is a logically plausible continuation of the prior reasoning and question context.
\end{itemize}

\paragraph{Justification.} This definition captures two core desiderata of a high-quality reasoning process: (1) \textit{stepwise coherence}, i.e., that each step $s_t$ logically follows from the prior reasoning $\mathbf{S}_{<t}$ and the question $q$, and (2) \textit{goal-directed correctness}, i.e., that each step contributes positively toward arriving at the correct final answer $A$. By taking the joint probability $P(A, s_t \mid \mathbf{S}_{<t}, q)$, we ensure that each step is evaluated not in isolation but in terms of both its contextual fit and its utility toward solving the task. Averaging over all steps distributes the credit across the reasoning trajectory, enabling a fine-grained assessment of reasoning quality at each point in the chain. This formulation is consistent with both causal and probabilistic perspectives, and provides a scalable, interpretable metric for assessing multi-step reasoning performance.


\subsection{Estimating Stepwise Coherence via Preference-Based Evaluation}

We aim to estimate $P(s_t \mid do(\mathbf{S}_{<t}), q)$, the plausibility of a reasoning step $s_t$ given the fixed prior chain $\mathbf{S}_{<t}$ and question $q$. Under the \textit{CoT Exogeneity} assumption, this is equivalent to computing the conditional likelihood $P(s_t \mid \mathbf{S}_{<t}, q)$. 

Rather than relying purely on language model log-probabilities, we adopt a preference-based evaluation approach to estimate this quantity more robustly. Specifically, we construct a set of contrastive candidate steps $\{s_t^{(j)}\}_{j=1}^k$ for each $s_t$, which represent plausible but logically imperfect alternatives that could reasonably occur under the same context $(\mathbf{S}_{<t}, q)$. These candidates simulate variations in the reasoning trajectory without altering the fixed prior steps — in analogy to sampling from a stochastic reasoning mechanism conditioned on the same history. We then prompt an external judge model (e.g., GPT-4) to compare $s_t$ against each contrastive: \yc{not an external judge model, just this model itself in our experiments.}

\begin{quote}
\texttt{Question: [q]} \\
\texttt{Previous reasoning: [$s_1$, ..., $s_{t-1}$]} \\
\texttt{Which of the following is a more logical next step?} \\
\texttt{Option A: [$s_t$]} \\
\texttt{Option B: [$s_t^{(j)}$]} \\
\texttt{Answer: [A/B/NA]}
\end{quote}

We define the stepwise coherence score as the fraction of contrastive comparisons in which $s_t$ is preferred:

\begin{equation}
\text{CoherenceScore}_t: \hat{P}(s_t \mid \mathbf{S}_{<t}, q)= \frac{\# \text{ correct preferences for } s_t}{\# \text{ total contrastive comparisons }}
\end{equation}

This coherence score serves as an empirical proxy for $P(s_t \mid \mathbf{S}_{<t}, q)$.

\paragraph{Contrastive candidate types.} 
To generate meaningful contrastive candidates, we design several types of contrastive candidates:
\begin{itemize}
\item Operation Error: Use wrong arithmetic/logic operation.
\item Conceptual Swap: Confuse formula components (radius vs. diameter, etc.)
\item Misgeneralization: Apply general rule incorrectly or heuristically.
\item Reordered Logic: Swap the logical sequence of sub-steps.
\item Contradiction: Assert facts that contradict prior steps
\end{itemize}
These contrastive steps are either generated by prompting the LLM with templated instructions (e.g., “introduce a small flaw in the reasoning”), or by applying predefined corruption heuristics to the gold step. By combining diverse error types, we ensure that $s_t$ is evaluated against a rich contrast space, better approximating $P(s_t \mid \mathbf{S}_{<t}, q)$ as a relative coherence likelihood.

\paragraph{Remark.} 
Although we do not access the full probabilistic space, we recover a normalized ranking over local support using human- or model-level judgments. This is particularly well-suited to evaluating reasoning chains in natural language, where coherence may not be easily captured by token-level likelihoods alone.



\subsection{Correctness Evaluation via Final Answer Likelihood}

The second term, $P(A \mid s_t, q)$, is evaluated by checking whether the step $s_t$ leads to the correct final answer (when composed with the remaining steps in the reasoning chain???). In practice, we evaluate this either via symbolic execution (e.g., math problem solving) or via prompting an LLM to judge whether $A$ logically follows from $s_t$ and $q$.

\subsection{Full Chain Evaluation}

Finally, we compute the chain-level score as the average of step-level joint probabilities:

\begin{equation}
P_{\text{CoT}}(\mathbf{S}) = \frac{1}{n} \sum_{t=1}^n P(A \mid s_t, q) \cdot \hat{P}(s_t \mid \mathbf{S}_{<t}, q)
\end{equation}

This framework allows us to attribute reasoning quality not just to final answers, but to the causal structure and coherence of intermediate steps in the reasoning process.



















==> main/method_final.tex <==
\section{The Basic Causal View}
To investigate the causal mechanisms underlying Chain-of-Thought (CoT) reasoning, we introduce a Structural Causal Model (SCM) and identify the LLM's parametric knowledge, denoted as \( Z \), as a key confounder. Figure 2a illustrates the SCM for conventional question-answering tasks. We further extend this framework to CoT prompting: Figure 2b presents the SCM when the CoT is treated as a single mediating variable \( S \), where the causal path \( Q \rightarrow S \rightarrow A \) indicates that the CoT mediates the relationship between the query and the answer. Figure 2c elaborates this view by decomposing the CoT into fine-grained steps. The causal path \( Q \rightarrow S_{\leq i} \rightarrow S_{> i} \rightarrow A \) allows us to estimate the causal effect of earlier steps \( S_{\leq i} \) on subsequent steps \( S_{> i} \). By systematically measuring this step-level causal effect across different segmentation points \( i \), we can quantitatively assess the strength of the logical connections between steps, thereby evaluating the overall coherence of the entire CoT.

We further present our proposed measurement for coherence , which incorporates an exogenous noise variable as an instrumental variable, in Figure 2d, and the details in \S\ref{coherence}. 
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{latex/imgs/graph.png}
    \caption{Causal Graph}
    \label{fig:causal_graph}
\end{figure}

\section{Methodology}
% \paragraph{Definition}
\subsection{CoT Reasoning Measurement}
% Requires: \usepackage{amsmath}
\paragraph{Definition 1.}
Given an input $Q=q$, the Chain-of-Thought~\citep{wei2023chainofthoughtpromptingelicitsreasoning} (CoT) reasoning process generates the final answer $A=a$ by sequentially deriving intermediate reasoning steps $\textbf{S}=\{s1,\ldots,s_i,\ldots,s_n\}$. The joint probability is:
\begin{equation}
\begin{aligned}
\nonumber
&P\big(A=a,\; \textbf{S}=\{s1,\ldots,s_i,\ldots,s_n\} \mid Q=q\big)\\
&= \underbrace{P\big(A=a \mid s_1,\ldots,s_n, q\big)}_{\text{Answer Correctness}}\cdot \underbrace{\prod_{i=1}^{n} P\big(s_i \mid s_{<i}, q\big)}_{\text{Chain Coherence}}.
\end{aligned}
\label{eq:cot_joint}
\end{equation}

\paragraph{Explanation.}
$P(A=a, \textbf{S} \mid Q=q)$ is the joint probability of generating the full reasoning trace $\textbf{S}$ and the final answer $a$. $P(a \mid s_1,\ldots,s_n, q)$ ($P_{\text{AC}}$) corresponds to the conditional probability of generating the final answer from the complete reasoning trace, while $\prod_{i=1}^{n} P(s_i \mid s_{<i}, q)$ ($P_{\text{CC}}$) models the sequential generation of the CoT steps.


\subsection{Answer Correctness ($P_{\text{AC}}$)}
Figure 2b illustrates the introduction of Chain-of-Thought (CoT) to guide the LLM through an explicit reasoning process before producing the final answer. The causal path \(Q \rightarrow S \rightarrow A\) indicates that the CoT \(S\) acts as a mediator between the query \(Q\) and the answer \(A\). In the general case where \(S\) is a stochastic mediator, the causal effect of \(Q\) on \(A\) is given by the mediation formula:
% \[
% P(A \mid do(Q=q)) = \sum_s P(A \mid do(Q=q), S=s) \cdot P(S=s \mid do(Q=q))
% \]
\begin{equation}
\begin{aligned}
\nonumber
P(A \mid do(Q=q)) = & \sum_s P(A \mid do(Q=q), S=s) \\ & \cdot P(S=s \mid do(Q=q))
\end{aligned}
\label{eq:cot_joint}
\end{equation}

In this work, however, we aim to estimate the causal effect on \(A\) when intervening on \(Q\) while fixing the CoT to a specific reasoning sequence \(\mathbf{s}\). This corresponds to the joint intervention \(do(Q=q, S=\mathbf{s})\), formalized as \(P(A \mid do(Q=q, S=\mathbf{s}))\). By constraining \(S\) to \(\mathbf{s}\), the conditional probability \(P(S=\mathbf{s} \mid do(Q=q))\) reduces to 1, collapsing the general mediation formula into a single term:
\begin{equation}
\begin{aligned}
\nonumber
P_{\text{AC}} & = P(A \mid do(Q=q, S=\mathbf{s})) \\ &= P(A \mid do(Q=q), S=\mathbf{s})
\end{aligned}
\label{eq:cot_joint}
\end{equation}

This simplification implies that, under the joint intervention fixing both \(Q = q\) and \(S = \mathbf{s}\), the causal effect is identified directly by the corresponding interventional distribution. This measure reflects the probability of the answer \(A\) when the model is compelled to use both the question \(q\) and the reasoning steps \(\mathbf{s}\), thereby providing a precise tool for evaluating the contribution of a reasoning path to answer correctness.


% We are interested in the causal effect of intervening on \( Q \) on the outcome \( A \), formally expressed as:
% \[
% P(A \mid do(Q=q))
% \]
% In the general case where \( S \) is a random variable, the back-door adjustment or mediation formula must be used:
% \begin{equation}
% \begin{aligned}
% \nonumber
% P(A \mid do(Q=q)) = & \sum_s P(A \mid do(Q=q), S=\textbf{S}) \\ & \cdot P(S=\textbf{S} \mid do(Q=q))
% \end{aligned}
% \label{eq:cot_joint}
% \end{equation}
% In our setting, \( S \) is fixed to a constant value \( \textbf{S} \), which used to measure the probability of such $\textbf{S}$, this implies: $P(S = \textbf{S} \mid do(Q=q)) = 1, P(S \neq\textbf{S}\mid do(Q=q)) = 0$. Consequently, the summation over all possible \( \textbf{S} \) collapses into a single term where \( S = \textbf{S} \):
% \[
% P(A \mid do(Q=q)) = P(A \mid do(Q=q), \textbf{S} = \textbf{s})
% \]
% This simplification means that, under the fixed \( S = \textbf{S}\) condition, the causal effect of \( Q \) on \( A \) is identified by the interventional distribution where both \( Q \) is set to \( q \) and \( S \) is set to \( \textbf{S} \).

\subsection{Chain Coherence ($P_{\text{CC}}$)}\label{coherence}
\paragraph{Causal Formulation}
In standard CoT reasoning, the causal path \(Q \rightarrow S_{\leq i} \rightarrow S_{> i} \rightarrow A\) suggests that early reasoning steps directly influence subsequent ones. However, this process may be confounded by unobserved factors, such as the LLM's internal parametric knowledge \(Z\), which could potentially influence multiple reasoning steps simultaneously, creating a risk of spurious association between \(S_{\leq i}\) and \(S_{> i}\).

To address this identification challenge and obtain a clean causal estimate, we introduce an exogenous instrumental variable \(U\), representing randomly assigned error types (e.g., logical fallacies, skipped steps). The variable \(U\) is independent of any confounders and is posited to influence \(S_{> i}\) only through its effect on \(S_{\leq i}\), thereby satisfying the key instrumental conditions. By intervening with \(U\), we generate exogenous variation in \(S_{\leq i}\), which allows us to identify the causal effect of early reasoning on subsequent reasoning quality without bias from unobserved common causes.

Let \(S = \{s_1, s_2, \ldots, s_n\}\) denote an arbitrary Chain-of-Thought (CoT) with \(n\) reasoning steps, and let \(\textbf{S}\) represent a specific given CoT. We partition the CoT at position \(i\):
- Early reasoning segment: \(S_{\leq i} = \{s_1, \ldots, s_i\}\)
- Subsequent reasoning segment: \(S_{> i} = \{s_{i+1}, \ldots, s_n\}\)

The corresponding causal graph is:
\(Q \rightarrow S_{\leq i} \rightarrow S_{> i} \rightarrow A, \quad U \rightarrow S_{\leq i}\).
We formalize the data-generating process through the following structural equations:

\[
\begin{aligned}
S_{\leq i} &:= g(Q, U) \\
S_{> i} &:= f(S_{\leq i}, Q)
\end{aligned}
\]

where \(U\) is an instrumental variable representing exogenous error types, \(g(\cdot)\) models the generation of early reasoning steps dependent on both the question \(Q\) and the instrumental variable \(U\), and \(f(\cdot)\) captures how **subsequent reasoning steps \(S_{> i}\) are generated based directly on the early steps \(S_{\leq i}\)** and the question context \(Q\).

The relationship between \(S_{\leq i}\) and \(U\) is explicitly defined through an error injection function. For a given original CoT segment \(\textbf{S}_{\leq i}\) and an error type \(u \in \mathcal{U}\):
\[
S_{\leq i}^{(u)} = \text{InjectError}(\textbf{S}_{\leq i}, u),
\]
where \(S_{\leq i}^{(\emptyset)}\) denotes the segment with no injected error (\(U = \emptyset\)).

\paragraph{Counterfactual Framework and ACE Definition}

Let \(S_{> i}^{(u)}\) denote the potential outcome of the subsequent reasoning segment under the intervention \(do(U=u)\). This represents the output of the function \(f(S_{\leq i}^{(u)}, Q)\), highlighting the direct dependency of \(S_{> i}\) on the intervened early segment \(S_{\leq i}^{(u)}\).

We aim to estimate the causal effect of variations in early reasoning (\(S_{\leq i}\)), induced by \(U\), on the quality of subsequent reasoning (\(S_{> i}\)). Formally, for a given error type \(u \in \mathcal{U}\), we define the individual-level causal effect:

\[
\text{ACE}(u) = \mathbb{E}\left[\phi\left(S_{> i}^{(\emptyset)}\right) - \phi\left(S_{> i}^{(u)}\right)\right]
\]

Under the instrumental variable assumptions, this simplifies to a contrast of conditional expectations:

\[
\text{ACE}(u) = \mathbb{E}\left[\phi(S_{> i}) \mid U=\emptyset, Q\right] - \mathbb{E}\left[\phi(S_{> i}) \mid U=u, Q\right]
\]

The overall Average Causal Effect (ACE) across all error types is then:

\begin{equation}
\begin{split}
P_{\text{CC}} = \widehat{\mathrm{ACE}} &= \frac{1}{|\mathcal{U}|} \sum_{u \in \mathcal{U}} \mathrm{ACE}(u) \\
&= \frac{1}{|\mathcal{U}|} \sum_{u \in \mathcal{U}} \left[ \phi(S_{> i}^{(\emptyset)}) - \phi(S_{> i}^{(u)}) \right]
\end{split}
\end{equation}

This estimator quantifies how much, on average, the quality of the subsequent reasoning \(\phi(S_{> i})\) changes when the early reasoning \(S_{\leq i}\) is perturbed by an exogenous error \(u \in \mathcal{U}\).

% Let \(S = \{s_1, s_2, \ldots, s_n\}\) denote an arbitrary Chain-of-Thought (CoT) with \(n\) reasoning steps, and let \(\textbf{S}\) represent a specific given CoT. We partition the CoT at position \(i\): Early reasoning segment: \(S_{\leq i} = \{s_1, \ldots, s_i\}\); Subsequent reasoning segment: \(S_{> i} = \{s_{i+1}, \ldots, s_n\}\)

% The corresponding causal graph is:
% $Q \rightarrow S_{\leq i} \rightarrow S_{> i} \rightarrow A, \quad U \rightarrow S_{\leq i}$. We formalize the data-generating process through the following structural equations:

% \[
% \begin{aligned}
% S_{> i} &:= f(S_{\leq i}, Q, U), \\
% % A &:= h(S_{> i}, Q)
% \end{aligned}
% \]
% where \(U\) is an instrumental variable representing exogenous error types, and \(f(\cdot)\) captures how subsequent reasoning steps are generated based on early steps \(S_{\leq i}\), question context \(Q\). Early steps \(S_{\leq i}\) dependent on the instrumental variable \(U\). The relationship between early reasoning steps $S_{\leq i}$ and the instrumental variable \(U\) is explicitly defined through the error injection function:
% \[
% S_{\leq i}^{(u)} = \text{InjectError}(\textbf{S}_{\leq i}, u),
% \]
% where \(\textbf{S}_{\leq i}\) is the original early segment of the given CoT \(\textbf{S}\), \(u \in {U}\) is a specific error type.


% \paragraph{Counterfactual Framework and ACE Definition}
% Let \(S_{> i}(\textbf{s})\) denote the potential outcome when we forcibly set \(S_{\leq i} = \textbf{s}\). We aim to estimate the causal effect of early reasoning quality on subsequent reasoning quality. Formally, for a given error type \(u \in U\), we define the individual-level causal effect:
% \begin{equation}
% \begin{aligned}
% \text{ACE}(u) = &\mathbb{E}[\phi(S_{> i}(f(S_{<=i},Q,\emptyset))) \\&- \phi(S_{> i}(f(S_{<=i},Q,u)))]
% \end{aligned}
% \end{equation}
% Under the instrumental variable assumptions, this simplifies to:

% \begin{equation}
% \begin{aligned}
%     \text{ACE}(u) = & \mathbb{E}[\phi(S_{> i}) \mid U=\emptyset, Q] \\ & - \mathbb{E}[\phi(S_{> i}) \mid U=u, Q]
% \end{aligned}
% \end{equation}
% The overall average causal effect across all error types is:
% \begin{equation}
% \begin{aligned}
% \widehat{\mathrm{ACE}} & = \mathbb{E}_{u \sim U}[\text{ACE}(u)] \\ & = \frac{1}{|{U}|}  \sum_{u \in {U}} \left[ \phi(S_{> i}^{}) - \phi(S_{> i}^{(u)}) \right]
% \end{aligned}
% \end{equation}

\subsection{Estimation}
How to estimate $\phi$.  

\subsection{Method}
Let $s{1:i}$ denote the sequence of intermediate reasoning steps generated by an LLM before step $i$, and $s{i+1:n}$ denote the subsequent steps. Our goal is to estimate the causal effect of $s{1:i}$ on $s{i+1:n}$ in the presence of confounding factors.

We introduce an instrumental variable $U \in \mathcal{E}$, where $U$ is sampled from a set of externally designed errors $\mathcal{E}$ (e.g., logical errors, skipped steps, etc.). For each prompt $x$, we intervene on the LLM to enforce $do(s_{1:i}=z)$ for some $z$ and simultaneously inject $U=u$ to obtain
\[
s_{i+1:n}^{(u)} = \text{LLM}(x,\ do(s_{1:i}=z),\ U=u).
\]
By construction, $U$ is independent of latent confounders affecting both $s_{1:i}$ and $s_{i+1:n}$, and only affects $s_{i+1:n}$ through $s_{1:i}$. This enables us to leverage $U$ as a valid instrument for causal effect estimation.


\subsection{Effect Estimation}

Let $Q(\cdot)$ denote a scoring function that quantifies the quality or correctness of the generated sequence $s{i+1:n}$ (e.g., by automated metrics or human evaluation). For a set of $m$ different instrument values $\{u1,\dots,um\}$ sampled from $\mathcal{E}$, we obtain corresponding outputs $\{s{i+1:n}^{(uj)}\}{j=1}^m$. For comparison, we also obtain outputs under the standard intervention (no error injected), denoted as $s_{i+1:n}^{(0)}$.

The average effect of $do(s_{1:i}=z)$ on $Q$ is then estimated by:
\[
\hat{\tau} = \frac{1}{m} \sum_{j=1}^{m} \left[ Q(s_{i+1:n}^{(0)}) - Q(s_{i+1:n}^{(uj)}) \right],
\]
where $\hat{\tau}$ yields an empirical measure of the marginal causal impact of modifying $s{1:i}$ (via $U$) on the quality of subsequent reasoning steps. This approach isolates exogenous variation in $s{1:i}$ induced by $U$, enabling unbiased estimation of its effect on downstream output through the LLM’s reasoning chain.

---
\subsection{Method}
To estimate the causal effect of early reasoning steps \( s_{\leq i} \) on the quality of subsequent steps \( s_{>i} \), we must account for unobserved confounders inherent in the LLM's generation process (e.g., internal biases, latent reasoning states). Directly correlating \( s_{\leq i} \) with \( s_{>i} \) yields a biased estimate. To overcome this, we employ an Instrumental Variables (IV) approach, leveraging a designed exogenous instrument \( U \).

Let:
- \( X \) be the treatment variable, representing the *potential realizations* of the subsequent steps \( s_{>i} \) generated from a given \( do(s_{\leq i}) \).
- \( Y \) be the outcome, representing the quality score of the generated \( s_{>i} \).
- \( U \) be our instrument, an exogenously imposed error (e.g., logical error, skipped step) on \( s_{\leq i} \).

A valid instrument \( U \) must satisfy three core conditions:
1.  Relevance: \( U \) is a cause of variation in the potential realizations of \( X \).
2.  Exclusion Restriction: \( U \) affects the outcome \( Y \) only through its effect on \( X \).
3.  Exogeneity: \( U \) is independent of unobserved confounders affecting \( Y \).

Our designed instrument \( U \), a randomly assigned synthetic error, satisfies these conditions by construction.

The structural model is defined as follows:

**First Stage (Generation of Subsequent Steps):**
The generation of the subsequent steps \( X \) is a function of the fixed initial steps and the instrument:
\[
X = f(do(s_{\leq i}), U) + \epsilon_1
\]
where \( f \) is the LLM's generation function, \( do(s_{\leq i}) \) is the fixed intervention, and \( U \) is the exogenous error. \( \epsilon_1 \) represents other unmodeled generation noise. This stage produces different potential realizations \( X(U) \) of the subsequent steps, driven solely by variations in \( U \).

**Second Stage (Quality Assessment):**
The quality \( Y \) of the generated steps \( X \) is given by:
\[
Y = \beta X + \epsilon_2
\]
where \( \beta \) is the causal effect of interest—the change in quality per unit change in the *potential realization* of the subsequent steps, induced by the instrument. \( \epsilon_2 \) contains all other factors affecting quality, including unobserved confounders.

The key insight is that by using \( U \) to generate variations in \( X \), we isolate a "clean" source of variation in the subsequent steps that is uncorrelated with the confounders in \( \epsilon_2 \).

---

### **4. Effect Estimation and Interpretation**

The causal effect \( \beta \) is estimated using the variations induced by the instrument \( U \). Let \( U = 0 \) represent the absence of an exogenous error (the original \( s_{\leq i} \)), and \( U = k \) represent the introduction of a specific error type \( k \).

For a given intervention \( do(s_{\leq i}) \), we generate:
- A reference output: \( X_0 = f(do(s_{\leq i}), U=0) \)
- A set of instrumented outputs: \( X_k = f(do(s_{\leq i}), U=k) \quad \forall k \in K \)

The quality of each generated sequence is then computed using an evaluation function \( \mathcal{Q} \):
\[
Y_0 = \mathcal{Q}(X_0), \quad Y_k = \mathcal{Q}(X_k)
\]

The causal effect of the early steps \( s_{\leq i} \) on the later steps, as mediated through the variation created by the instrument, can be estimated for each error type \( k \) as the Intent-to-Treat (ITT) effect:
\[
\text{ITT}_k = Y_k - Y_0
\]
This represents the change in final output quality attributable to the introduction of error \( k \) in the early steps.

To aggregate these into a single overall causal effect estimate \( \hat{\beta}_{IV} \) for the \( do(s_{\leq i}) \) intervention, we use the following ratio, which is the standard IV estimator in a multi-valued instrument setting:
\[
\hat{\beta}_{IV} = \frac{\mathbb{E}[Y | do(s_{\leq i}), U] - Y_0}{\mathbb{E}[X | do(s_{\leq i}), U] - X_0} \approx \frac{\frac{1}{|K|}\sum_{k=1}^{|K|} (Y_k - Y_0)}{\frac{1}{|K|}\sum_{k=1}^{|K|} \mathcal{D}(X_k, X_0)}
\]
Here, \( \mathcal{D}(X_k, X_0) \) is a semantic or syntactic distance metric (e.g., BLEU score, edit distance, embedding cosine distance) that quantifies the divergence between the instrumented output \( X_k \) and the reference output \( X_0 \). The numerator is the average change in quality, and the denominator is the average induced change in the subsequent steps' content. The ratio \( \hat{\beta}_{IV} \) thus estimates the average causal effect of the early steps on the quality of the later steps per unit of instrument-induced change, providing a consistent estimate of the parameter \( \beta \) in the structural model.

---

\subsection{Causal Formulation of Reasoning Step Quality}

We model reasoning as a sequential generative process governed by a structural causal model (SCM), under which the reasoning chain is conceptualized as a causal sequence. Each reasoning step $s_t$ is generated by a deterministic structural equation:

\begin{equation}
s_t = f_t(s_{<t}, q, U_t)
\end{equation}
with $U_t$ denoting an exogenous noise variable. 
To evaluate whether a given step is plausible given the prior reasoning, we assess the interventional probability $P(s_t \mid do(s_{<t}), q)$, representing the likelihood of $s_t$ under a fixed prefix of reasoning. 

\paragraph{CoT Exogeneity Assumption.} We assume that reasoning step generation is conditionally exogenous: it depends only on the prior steps and the question, not on hidden variables. Formally:
\begin{equation}
P(s_t \mid do(s_{<t}), q) = P(s_t \mid s_{<t}, q)
\end{equation}

This allows us to approximate step plausibility via standard conditional language model probabilities. %We define the overall chain-of-thought quality score as:
% \begin{equation}
% P_{\text{CoT}}(\mathbf{S}) = \frac{1}{n} \sum_{t=1}^n P(A \mid s_t, q) \cdot P(s_t \mid s_{<t}, q)
% \end{equation}


\subsection{Quantifying Reasoning Quality with \texorpdfstring{$P_{\text{CoT}}$}{PCoT}}

We define the quality of a reasoning chain $\mathbf{S} = \{s_1, s_2, \dots, s_n\}$ for a given question $q$ through the metric $P_{\text{CoT}}$, which captures whether each reasoning step $s_t$ contributes to both accurate continuation and correctness of the final answer $A$. Formally, we define:

\begin{definition}[$P_{\text{CoT}}$] The high-quality reasoning chain $\mathbf{S} = \{s_1, \dots, s_n\}$ is one where each step $s_t$ accurately predicts the next step $s_{t+1}$ and contributes to the correct final answer. This can be quantified using Bayesian probability:
\begin{equation}
P_{\text{CoT}}(\mathbf{S}) = \frac{1}{n} \sum_{t=1}^n P(A, s_t \mid \mathbf{S}_{<t}, q),
\end{equation}
where $A$ is the correct answer, $q$ is the input question, and $\mathbf{S}_{<t} = \{s_1, \dots, s_{t-1}\}$.
\end{definition}

Applying Bayes’ rule, we decompose this joint probability into two interpretable components:

\begin{equation}
P_{\text{CoT}}(s_t) = P(A, s_t \mid \mathbf{S}_{<t}, q) = P(A \mid s_t, q) \cdot P(s_t \mid do(\mathbf{S}_{<t}), q)
\end{equation}

This formulation allows us to isolate two critical aspects of reasoning:
\begin{itemize}
    \item \textbf{Correctness Term} ($P(A \mid s_t, q)$): Measures whether the step $s_t$ contributes to the correct final answer $A$.
    \item \textbf{Coherence Term} ($P(s_t \mid do(\mathbf{S}_{<t}), q)$): Captures whether $s_t$ is a logically plausible continuation of the prior reasoning and question context.
\end{itemize}

\paragraph{Justification.} This definition captures two core desiderata of a high-quality reasoning process: (1) \textit{stepwise coherence}, i.e., that each step $s_t$ logically follows from the prior reasoning $\mathbf{S}_{<t}$ and the question $q$, and (2) \textit{goal-directed correctness}, i.e., that each step contributes positively toward arriving at the correct final answer $A$. By taking the joint probability $P(A, s_t \mid \mathbf{S}_{<t}, q)$, we ensure that each step is evaluated not in isolation but in terms of both its contextual fit and its utility toward solving the task. Averaging over all steps distributes the credit across the reasoning trajectory, enabling a fine-grained assessment of reasoning quality at each point in the chain. This formulation is consistent with both causal and probabilistic perspectives, and provides a scalable, interpretable metric for assessing multi-step reasoning performance.


\subsection{Estimating Stepwise Coherence via Preference-Based Evaluation}

We aim to estimate $P(s_t \mid do(\mathbf{S}_{<t}), q)$, the plausibility of a reasoning step $s_t$ given the fixed prior chain $\mathbf{S}_{<t}$ and question $q$. Under the \textit{CoT Exogeneity} assumption, this is equivalent to computing the conditional likelihood $P(s_t \mid \mathbf{S}_{<t}, q)$. 

Rather than relying purely on language model log-probabilities, we adopt a preference-based evaluation approach to estimate this quantity more robustly. Specifically, we construct a set of contrastive candidate steps $\{s_t^{(j)}\}_{j=1}^k$ for each $s_t$, which represent plausible but logically imperfect alternatives that could reasonably occur under the same context $(\mathbf{S}_{<t}, q)$. These candidates simulate variations in the reasoning trajectory without altering the fixed prior steps — in analogy to sampling from a stochastic reasoning mechanism conditioned on the same history. We then prompt an external judge model (e.g., GPT-4) to compare $s_t$ against each contrastive: \yc{not an external judge model, just this model itself in our experiments.}

\begin{quote}
\texttt{Question: [q]} \\
\texttt{Previous reasoning: [$s_1$, ..., $s_{t-1}$]} \\
\texttt{Which of the following is a more logical next step?} \\
\texttt{Option A: [$s_t$]} \\
\texttt{Option B: [$s_t^{(j)}$]} \\
\texttt{Answer: [A/B/NA]}
\end{quote}

We define the stepwise coherence score as the fraction of contrastive comparisons in which $s_t$ is preferred:

\begin{equation}
\text{CoherenceScore}_t: \hat{P}(s_t \mid \mathbf{S}_{<t}, q)= \frac{\# \text{ correct preferences for } s_t}{\# \text{ total contrastive comparisons }}
\end{equation}

This coherence score serves as an empirical proxy for $P(s_t \mid \mathbf{S}_{<t}, q)$.

\paragraph{Contrastive candidate types.} 
To generate meaningful contrastive candidates, we design several types of contrastive candidates:
\begin{itemize}
\item Operation Error: Use wrong arithmetic/logic operation.
\item Conceptual Swap: Confuse formula components (radius vs. diameter, etc.)
\item Misgeneralization: Apply general rule incorrectly or heuristically.
\item Reordered Logic: Swap the logical sequence of sub-steps.
\item Contradiction: Assert facts that contradict prior steps
\end{itemize}
These contrastive steps are either generated by prompting the LLM with templated instructions (e.g., “introduce a small flaw in the reasoning”), or by applying predefined corruption heuristics to the gold step. By combining diverse error types, we ensure that $s_t$ is evaluated against a rich contrast space, better approximating $P(s_t \mid \mathbf{S}_{<t}, q)$ as a relative coherence likelihood.

\paragraph{Remark.} 
Although we do not access the full probabilistic space, we recover a normalized ranking over local support using human- or model-level judgments. This is particularly well-suited to evaluating reasoning chains in natural language, where coherence may not be easily captured by token-level likelihoods alone.



\subsection{Correctness Evaluation via Final Answer Likelihood}

The second term, $P(A \mid s_t, q)$, is evaluated by checking whether the step $s_t$ leads to the correct final answer (when composed with the remaining steps in the reasoning chain???). In practice, we evaluate this either via symbolic execution (e.g., math problem solving) or via prompting an LLM to judge whether $A$ logically follows from $s_t$ and $q$.

\subsection{Full Chain Evaluation}

Finally, we compute the chain-level score as the average of step-level joint probabilities:

\begin{equation}
P_{\text{CoT}}(\mathbf{S}) = \frac{1}{n} \sum_{t=1}^n P(A \mid s_t, q) \cdot \hat{P}(s_t \mid \mathbf{S}_{<t}, q)
\end{equation}

This framework allows us to attribute reasoning quality not just to final answers, but to the causal structure and coherence of intermediate steps in the reasoning process.


















